Multi-clue reconstruction of sharing chains for social media images

The amount of multimedia content shared everyday, combined with the level of realism reached by recent fake-generating technologies, threatens to impair the trustworthiness of online information sources. The process of uploading and sharing data tends to hinder standard media forensic analyses, since multiple re-sharing steps progressively hide the traces of past manipulations. At the same time though, new traces are introduced by the platforms themselves, enabling the reconstruction of the sharing history of digital objects, with possible applications in information flow monitoring and source identification. In this work, we propose a supervised framework for the reconstruction of image sharing chains on social media platforms. The system is structured as a cascade of backtracking blocks, each of them tracing back one step of the sharing chain at a time. Blocks are designed as ensembles of classifiers trained to analyse the input image independently from one another by leveraging different feature representations that describe both content and container of the media object. Individual decisions are then properly combined by a late fusion strategy. Results highlight the advantages of employing multiple clues, which allow accurately tracing back up to three steps along the sharing chain.

==> tabs/cascade-step-2-results.tex <==
\begin{table}[htbp!]
\centering
\begin{tabular}{lcccc}
\toprule
Sharing chain & Accuracy & Sensitivity & Specificity & Precision \\
\midrule
FB & 0.9748 & 0.8313 & 0.9792 & 0.5542 \\
FB-FB & 0.9695 & 0.0000 & 1.0000 & 0.0000 \\
FB-FB-FB & 0.9626 & 0.8698 & 0.9655 & 0.4441 \\
FL-FB-FB & 0.9915 & 0.8024 & 0.9974 & 0.9054 \\
TW-FB-FB & 0.9924 & 0.7574 & 0.9983 & 0.9196 \\
FL-FB & 0.9697 & 0.3245 & 0.9879 & 0.4298 \\
FB-FL-FB & 0.9695 & 0.3529 & 0.9871 & 0.4390 \\
FL-FL-FB & 0.9691 & 0.7862 & 0.9746 & 0.4789 \\
TW-FL-FB & 0.9842 & 0.7590 & 0.9912 & 0.7283 \\
TW-FB & 0.9902 & 0.0000 & 1.0000 & 0.0000 \\
FB-TW-FB & 0.9804 & 0.4923 & 0.9922 & 0.6038 \\
FL-TW-FB & 0.9742 & 0.5057 & 0.9817 & 0.3077 \\
TW-TW-FB & 0.9902 & 0.0000 & 1.0000 & 0.0000 \\
\midrule
FL & 0.9835 & 0.6170 & 0.9931 & 0.7016 \\
FB-FL & 0.9757 & 0.2727 & 0.9944 & 0.5652 \\
FB-FB-FL & 0.9713 & 0.4648 & 0.9847 & 0.4459 \\
FL-FB-FL & 0.9891 & 0.9367 & 0.9907 & 0.7475 \\
TW-FB-FL & 0.9600 & 0.9051 & 0.9617 & 0.4109 \\
FL-FL & 0.9875 & 0.8833 & 0.9910 & 0.7681 \\
FB-FL-FL & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
FL-FL-FL & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
TW-FL-FL & 0.9875 & 0.7333 & 0.9961 & 0.8627 \\
TW-FL & 0.9702 & 0.2044 & 0.9898 & 0.3373 \\
FB-TW-FL & 0.9699 & 0.0000 & 0.9996 & 0.0000 \\
FL-TW-FL & 0.9640 & 0.7162 & 0.9709 & 0.4046 \\
TW-TW-FL & 0.9679 & 0.2029 & 0.9875 & 0.2947 \\
\midrule
TW & 0.9913 & 0.0000 & 1.0000 & 0.0000 \\
FB-TW & 0.9577 & 0.3012 & 0.9781 & 0.2994 \\
FB-FB-TW & 0.9546 & 0.3095 & 0.9749 & 0.2796 \\
FL-FB-TW & 0.9526 & 0.9458 & 0.9528 & 0.3839 \\
TW-FB-TW & 0.9893 & 0.8444 & 0.9942 & 0.8306 \\
FL-TW & 0.9713 & 0.2066 & 0.9885 & 0.2874 \\
FB-FL-TW & 0.9788 & 0.3533 & 0.9983 & 0.8676 \\
FL-FL-TW & 0.9791 & 0.2240 & 0.9967 & 0.6087 \\
TW-FL-TW & 0.9798 & 0.8222 & 0.9852 & 0.6520 \\
TW-TW & 0.9916 & 0.0000 & 1.0000 & 0.0000 \\
FB-TW-TW & 0.9699 & 0.0000 & 1.0000 & 0.0000 \\
FL-TW-TW & 0.9408 & 0.5041 & 0.9506 & 0.1865 \\
TW-TW-TW & 0.9916 & 0.0000 & 1.0000 & 0.0000 \\
\bottomrule
\end{tabular}
\caption{Reconstruction of the complete sharing chain ($[C_{-2},C_{-1},C_0]$) with all feature descriptors (DCT, META, HEADER); overall accuracy = 0.5465 (random guess = 0.0256); overall rejection rate = 0.1949.}
\end{table}
